Stability Properties of Graph Neural Networks

Graph neural networks (GNNs) have emerged as a powerful tool for nonlinear processing of graph signals, exhibiting success in recommender systems, power outage prediction, and motion planning, among others. GNNs consists of a cascade of layers, each of which applies a graph convolution, followed by a pointwise nonlinearity. In this work, we study the impact that changes in the underlying topology have on the output of the GNN. First, we show that GNNs are permutation equivariant, which implies that they effectively exploit internal symmetries of the underlying topology. Then, we prove that graph convolutions with integral Lipschitz filters, in combination with the frequency mixing effect of the corresponding nonlinearities, yields an architecture that is both stable to small changes in the underlying topology and discriminative of information located at high frequencies. These are two properties that cannot simultaneously hold when using only linear graph filters, which are either discriminative or stable, thus explaining the superior performance of GNNs.

==> figures/figGraphScatteringTransform.tex <==
%!TEX root = ../stability.tex

\def \thisplotscale {1}

\def \unit {\thisplotscale cm}

\tikzstyle {node} = 
	[circle, 
	 draw,
	 minimum width = 0.25*\unit,
	 minimum height = 0.25*\unit,
	 anchor = center]
     
\def\colorNode{pennblue}
\def\colorEdge{penndarkestblue}
\def\colorGraphFilter{pennlightestblue}
\def\colorSummarizer{pennlightestred}
\def\colorBinding{pennmediumgray1}

\def\dist{1.5}

\def\xlbl{0.1*\dist}
\def\ylbl{0.1*\dist}

\def\myLineWidth{1.25}
\def\myArrowWidth{2}
\def\angleSummarizer{160}
\def\radiusSummarizer{1.5}
\def\shortsize{10}

\def\halfImageWidth{8*\unit}
\def\distBetweenLayers{0.414*\halfImageWidth}
\def\distNodesLayerOne{0.42*\halfImageWidth}
\def\distNodesLayerTwo{0.225*\distNodesLayerOne}

{\footnotesize \begin{tikzpicture}[x = 1*\unit, y = 1*\unit]
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % Define anchor points
    % Origin point
	\node at (0, 0) (o) {};
    % Zeroth layer
    \path (o) ++ (-\halfImageWidth,0)
                    node (leftEdgeLayer0) {};
    \path (o) ++ (\halfImageWidth,0)
                    node (rightEdgeLayer0) {};
    % First layer
    \path (o) ++ (-\halfImageWidth,-\distBetweenLayers)
                    node (leftEdgeLayer1) {};
    \path (o) ++ (\halfImageWidth,-\distBetweenLayers)
                    node (rightEdgeLayer1) {};
    % Second layer
    \path (o) ++ (-\halfImageWidth,-2*\distBetweenLayers)
                    node (leftEdgeLayer2) {};
    \path (o) ++ (\halfImageWidth,-2*\distBetweenLayers)
                    node (rightEdgeLayer2) {};   
    
    % Layer lines
    \draw [draw=\colorEdge, line width = \myLineWidth] 
          (leftEdgeLayer0) -- (rightEdgeLayer0);
    \draw [draw=\colorEdge, line width = \myLineWidth] 
          (leftEdgeLayer1) -- (rightEdgeLayer1);
    \draw [draw=\colorEdge, line width = \myLineWidth] 
          (leftEdgeLayer2) -- (rightEdgeLayer2);
    
	% Draw nodes
    % Zeroth layer nodes
	\path (o) 
		      node (0) [fill = \colorNode, node, draw = \colorEdge] {};
    % First layer nodes
    \path (0) ++ (-1.5*\distNodesLayerOne,-\distBetweenLayers)
              node (1) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (0) ++ (-0.5*\distNodesLayerOne,-\distBetweenLayers)
              node (2) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (0) ++ (0.5*\distNodesLayerOne,-\distBetweenLayers)
              node (3) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (0) ++ (1.5*\distNodesLayerOne,-\distBetweenLayers)
              node (4) [fill = \colorNode, node, draw = \colorEdge] {};
    % Second layer nodes
    %   From first node
    \path (1) ++ (-1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (11) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (1) ++ (-0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (12) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (1) ++ (0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (13) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (1) ++ (1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (14) [fill = \colorNode, node, draw = \colorEdge] {};
    %   From second node
    \path (2) ++ (-1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (21) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (2) ++ (-0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (22) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (2) ++ (0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (23) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (2) ++ (1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (24) [fill = \colorNode, node, draw = \colorEdge] {};
    %   From third node
    \path (3) ++ (-1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (31) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (3) ++ (-0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (32) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (3) ++ (0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (33) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (3) ++ (1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (34) [fill = \colorNode, node, draw = \colorEdge] {};
    %   From fourth node
    \path (4) ++ (-1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (41) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (4) ++ (-0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (42) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (4) ++ (0.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (43) [fill = \colorNode, node, draw = \colorEdge] {};
    \path (4) ++ (1.5*\distNodesLayerTwo,-\distBetweenLayers)
              node (44) [fill = \colorNode, node, draw = \colorEdge] {};
              
    % Graph filtering arrows
    %   Between Layer 0 and Layer 1
    \path (0.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node [above left, pos = 0.666] {$\bbH_{1}$} (1.north east);
    \path (0.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node [above left, pos = 0.666] {$\bbH_{2}$} (2.north);
    \path (0.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node [above right, pos = 0.666] {$\bbH_{3}$} (3.north);
    \path (0.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node [above right, pos = 0.666] {$\bbH_{4}$} (4.north west);
    %   Between Layer 1 and Layer 2
    %       For first element
    \path (1.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (11.north east);
    \path (1.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (12.north);
    \path (1.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (13.north);
    \path (1.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (14.north west);
    %       For second element
    \path (2.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (21.north east);
    \path (2.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (22.north);
    \path (2.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (23.north);
    \path (2.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (24.north west);
    %       For third element
    \path (3.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (31.north east);
    \path (3.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (32.north);
    \path (3.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (33.north);
    \path (3.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (34.north west);
    %       For fourth element
    \path (4.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (41.north east);
    \path (4.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (42.north);
    \path (4.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (43.north);
    \path (4.south) 
       edge [draw = \colorGraphFilter, line width = \myArrowWidth, -stealth] 
       node {} (44.north west);
    % Summarizer operations
    %   Zeroth Layer
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (0.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [above right] {$\phi_{(0)}(\bbx)$};
    %   First Layer
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (1.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [above right] {$\phi_{(1)}(\bbx)$};
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (2.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [above right] {$\phi_{(2)}(\bbx)$};
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (3.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [above] {$\phi_{(3)}(\bbx)$};
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (4.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [left] {$\phi_{(4)}(\bbx)$};
    %   Second Layer
    \draw [draw = \colorSummarizer, line width = \myArrowWidth, -stealth]
        (11.north west) -- + (\angleSummarizer:\radiusSummarizer)
        node [above right] {$\phi_{(1,1)}(\bbx)$};
        
        
    % Labeling
    %   Layers
    \node at (rightEdgeLayer0) [right] {$\ell=0$};
    \node at (rightEdgeLayer1) [right] {$\ell=1$};
    \node at (rightEdgeLayer2) [right] {$\ell=2=L$};
    %   Layer outputs
    \node at (leftEdgeLayer0) [left] {\color{\colorNode} $\bbx^{(0)}$};
    \node at (leftEdgeLayer1) [left] {\color{\colorNode} $\bbx^{(1)}$};
    \node at (leftEdgeLayer2) [left] {\color{\colorNode} $\bbx^{(2)}$};
    %   Nodes
    %       Zeroth layer
    \node at (0.north east) [above right] {$\bbx_{(0)} = \bbx$};
    %       First layer
    \node at (1.north west) [above] {$\bbx_{(1)}$};
    \node at (2.north east) [above right] {$\bbx_{(2)}$};
    \node at (3.north east) [above right] {$\bbx_{(3)}$};
    \node at (4.north east) [above] {$\bbx_{(4)}$};
    %       Second layer
    \node at (11.south) [below] {$\bbx_{(1,1)}$};
    \node at (12.south) [below] {$\bbx_{(1,2)}$};
    \node at (13.south) [below] {$\bbx_{(1,3)}$};
    \node at (14.south) [below] {$\bbx_{(1,4)}$};
    \node at (21.south) [below] {$\bbx_{(2,1)}$};
    \node at (22.south) [below] {$\bbx_{(2,2)}$};
    \node at (23.south) [below] {$\bbx_{(2,3)}$};
    \node at (24.south) [below] {$\bbx_{(2,4)}$};
    \node at (31.south) [below] {$\bbx_{(3,1)}$};
    \node at (32.south) [below] {$\bbx_{(3,2)}$};
    \node at (33.south) [below] {$\bbx_{(3,3)}$};
    \node at (34.south) [below] {$\bbx_{(3,4)}$};
    \node at (41.south) [below] {$\bbx_{(4,1)}$};
    \node at (42.south) [below] {$\bbx_{(4,2)}$};
    \node at (43.south) [below] {$\bbx_{(4,3)}$};
    \node at (44.south) [below] {$\bbx_{(4,4)}$};
    
    % Filters all-together
    \draw [draw = \colorBinding, line width = \myLineWidth] 
        (1) + (0, 0.5 * \distBetweenLayers) arc (100:80:29) 
        node [above right] {$\ccalH_{J}^{(1)} = \ccalH_{J} = \ccalH_{4}$};
    \draw [draw = \colorBinding, line width = \myLineWidth] 
        (11) + (0, 0.25 * \distBetweenLayers) arc (100:80:6.5) 
        node [above right] {$\ccalH_{J}$};
    \draw [draw = \colorBinding, line width = \myLineWidth] 
        (11) + (0, 0.5 * \distBetweenLayers) arc (100:80:35.5) 
        node [above right] {$\ccalH_{J}^{(2)}$};
    
    
        
%	\draw [draw = \colorfilteronetwotwo, line width = 0.75*\myLineWidth, -stealth] (h123.south) -- (h125.south);
	
\end{tikzpicture}} 


==> figures/tikz_styles.tex <==
\tikzstyle{phantom vertex} = [ ellipse, 
                               anchor = center, 
                               minimum height = 0.06*\unit, 
                               minimum width  = 0.06*\unit,
                               inner sep=0pt,
                               anchor=center]
\tikzstyle{red vertex}   = [black, fill = red!20,   phantom vertex, draw]
\tikzstyle{black vertex} = [black, fill = black!20, phantom vertex, draw]
\tikzstyle{blue vertex}  = [black, fill = blue!20,  phantom vertex, draw]
\tikzstyle{green vertex} = [black, fill = green!20,  phantom vertex, draw]
\tikzstyle{vertex}       = [draw, phantom vertex]

\tikzstyle{point} = [ellipse, inner sep=0pt, draw, fill=white, anchor = center,
                     minimum height = 0.05*\unit, minimum width  = 0.05*\unit]

==> graphNeuralNetworks.tex <==
%!TEX root = stability.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SECTION : Graph Neural Networks  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stability Properties of\\Graph Neural Networks} \label{sec:graphNeuralNetworks}

The superior performance of graph neural networks (GNNs) can be explained by the use of filter banks and nonlinearities to successfully process high-eigenvalue frequencies in a stable manner. An arbitrary GNN $\Phi(\bbS, \cdot)$ with $L$ layers, over a graph representation $\bbS$, is defined by \eqref{eqn_gnn_filter}-\eqref{eqn_gnn_nonlinearity} for $\ell=1,\ldots,L$. GNNs retain the two fundamental properties of linear filters. Namely, that they are permutation equivariant, and that they are stable.

%%%%%%%%%%%%%%
% PROPOSITION: prop:GNNPermutationEquivariance
%%%%%%%%%%%%%%
%
\begin{proposition}[GNN permutation equivariance] \label{prop:GNNPermutationEquivariance}
Consider graph shifts $\bbS$ and $\hbS = \bbP^{\Tr} \bbS \bbP$ for some permutation matrix $\bbP \in \ccalP$ [cf. \eqref{eqn:permutationSet}]. Given a bank of filters $\{\bbh_{\ell}^{fg}\}$ for each layer $\ell=1,\ldots,L$ and a pointwise nonlinearity $\sigma$, define a GNN $\Phi$ [cf. \eqref{eqn_gnn_filter}-\eqref{eqn_gnn_nonlinearity}]. Then, for any pair of corresponding graph signals $\bbx$ and $\hbx = \bbP^{\Tr} \bbx$ used as input to the GNN it holds that
% eqn
\begin{equation}
\Phi(\hbS, \hbx) = \bbP^{\Tr} \Phi(\bbS, \bbx).
\end{equation}
%
\end{proposition}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
See Appendix~\ref{sec_apx_D}.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

The stability of GNNs is inherited from the stability of the graph filters that conform the filter bank used in \eqref{eqn_gnn_filter}. The details of the GNN architecture control how this stability propagates.

%%%%%%%%%%
% THEOREM: thm:GNNStability
%%%%%%%%%%
%
\begin{theorem}[GNN Stability] \label{thm:GNNStability}
Let $\bbS$ and $\hbS$ be GSOs related by perturbation matrix $\bbE$ [cf. \eqref{eqn_def_operator_distance_error_matrix} or \eqref{eqn_relative_perturbation_distance}] such that $\| \bbE \| \leq \varepsilon$. Given a bank of filters $\{\bbh_{\ell}^{fg}\}$ such that $|h_{\ell}^{fg}(\lambda)| \leq 1$ [cf. \eqref{eqn_gnn_section_frequency_response}] and a pointwise nonlinearity $\sigma$ that is Lipschitz continuous \eqref{eqn_Lipschitz_nonlinearity}, define GNNs $\Phi(\bbS, \cdot)$ and $\Phi(\hbS, \cdot)$ [cf. \eqref{eqn_gnn_filter}-\eqref{eqn_gnn_nonlinearity}]. If the corresponding filter banks satisfy $\| \bbH_{\ell}^{fg}(\bbS) - \bbH_{\ell}^{fg}(\hbS) \|_{\ccalP} \leq \Delta \varepsilon$, then it holds that
%
\begin{equation}
    \| \Phi(\bbS, \cdot) - \Phi(\hbS, \cdot) \|_{\ccalP} \leq \Delta LF^{L-1} \varepsilon + \ccalO(\varepsilon^{2})
\end{equation}
%
for a GNN with a single input feature, a single output feature and $F$ features in each hidden layer.
\end{theorem}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
See Appendix \ref{sec_apx_E}.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

Thm.~\ref{thm:GNNStability} establishes how the stability of the filters $\Delta$ is affected by the hyperparameters of the GNN architecture. More specifically, we see that the stability gets degraded linearly with the number of layers $L$, and exponentially with the number of features $F$ (with an exponent controlled by $L$). In essence, the deeper a GNN is, the less stable it is. However, we see that the result is still linear in the size of the perturbation $\varepsilon$ and in the stability constant $\Delta$ of the filters. This stability constant depends on the perturbation model under consideration (either absolute --Sec.~\ref{sec_graph_perturbations}-- or relative --Sec.~\ref{sec_graph_perturbations_relative}--) and on the Lipschitz condition on the graph filters (either Lipschitz --Def.~\ref{def:lipschitzFilters}-- or integral Lipschitz --Def.~\ref{def:integralLipschitzFilters}--), as determined next.

%%%%%%%%%%%%%%
% PROPOSITION: prop:GNNPermutationEquivariance
%%%%%%%%%%%%%%
%
\begin{proposition}\label{prop:Delta}
Under the conditions of Thm.~\ref{thm:GNNStability}, with $\bbS = \bbV \bbLambda \bbV^{\Hr}$, consider the following models.
%
\begin{enumerate}[(i)]
    \vspace{.2cm}
%    
    \item If matrix $\bbE = \bbU \bbM \bbU^{\Hr}$ models absolute perturbations [cf. \eqref{eqn_def_operator_distance_error_matrix}], and the filters are Lipschitz (Def.~\ref{def:lipschitzFilters}) we have
    \begin{equation}
    \bbDelta = C (1+\delta \sqrt{N})
    \end{equation}
    with $\delta = (\| \bbU - \bbV \| + 1)^{2}-1$.
%    
    \vspace{.4cm}
%    
    \item If matrix $\bbE = \bbU \bbM \bbU^{\Hr}$ models relative perturbations (Def.~\ref{def_relative_perturbation}), and the filters are integral Lipschitz (Def.~\ref{def:integralLipschitzFilters}),
    \begin{equation}
    \bbDelta = 2 C (1+\delta \sqrt{N})
    \end{equation}
    holds with $\delta = (\| \bbU - \bbV \| + 1)^{2}-1$.
%    
    \vspace{.4cm}
%    
    \item If matrix $\bbE$ models relative perturbations (Def.~\ref{def_relative_perturbation}) and satisfies \eqref{eqn:structuralConstraint}, and the filters are integral Lipschitz (Def.~\ref{def:integralLipschitzFilters}),
    \begin{equation}
    \bbDelta = 2C.
    \end{equation}
%    
\end{enumerate}
%
\end{proposition}
%
%%%%%%%%%
%% Proof:
%%%%
%
\begin{proof}
Follows directly from Thm.~\ref{thm:GNNStability} in combination with Thms.~\ref{thm:filterStabilityAbsolute},~\ref{thm:filterStabilityRelative}~and~\ref{thm_filter_stability_structural_constraint}. These theorems establish the conditions and the corresponding values of $\Delta$.
\end{proof}
%
%% End of Proof
%%%%%%%%%%%%%%%%

The results of Thm.~\ref{thm:GNNStability} in combination with Prop.~\ref{prop:Delta} show that: (i) the use of Lipschitz filters lead to stable GNNs under absolute perturbations, and (ii) the use of integral Lipschitz filters lead to stable GNNs under relative perturbations. In all cases, Thm.~\ref{thm:GNNStability} establishes that GNNs $\bbPhi(\bbS, \bbx)$ are Lipschitz stable with respect to $\bbS$ (i.e., it does not establish Lipschitz stability with respect to $\bbx$).

The value of $\varepsilon$ in model (i) of Prop.~\ref{prop:Delta} represents the absolute perturbation distance (cf.~Def~\ref{def_operator_distance}) between shifts $\bbS$ and $\hbS$ and as such, is independent of the actual particularities of the graph under study (a fixed value of $\varepsilon$ would mean a different perturbation level for graphs that have very different edge weights). Likewise, the value of $C$ is given by the Lipschitz constant of the filters. The higher the value of $C$, the more selective the filters can be (the more narrow they can be), but the more unstable the GNNs become. Finally, the value of $\delta$ accounts for the eigenvector misalignment between the absolute error matrix $\bbE$ and the shift $\bbS$, which indicates the impact on the spectrum basis by the perturbation, and affects the stability bound by a value dependent on the number of nodes (the larger the graph, the more a change in the spectrum basis affects stability).

With respect to model (ii) of Prop.~\ref{prop:Delta} we observe that now $\varepsilon$ represents the relative distance between $\bbS$ and its perturbation $\hbS$ [cf.~\eqref{eqn_relative_perturbation_distance}], meaning that a fixed $\varepsilon$ represents the same level of perturbation for any possible reweighing of the difference $\alpha (\bbS - \hbS)$, $\alpha \in \reals$. The value of $C$, in this case, represents the integral Lipschitz constant of the filters (cf.~Def.~\ref{def:integralLipschitzFilters}). Integral Lipschitz filters, however, can be made arbitrarily selective near $\lambda \approx 0$, irrespective of the value of $C$, allowing for perfect discrimination of features around it, without affecting the overall stability. In integral Lipschitz filters, the value of $C$ determines the smallest eigenvalue for which the filter response becomes (approximately) flat, and hence loses discriminative power. A high value of $C$ would allow for greater selectivity in higher-eigenvalue frequencies, but at the expense of stability. With respect to $\delta$, the same analysis as for model (i) holds, except that in this case, the eigenvectors $\bbU$ correspond to the \emph{relative} error matrix $\bbE$.

To overcome the degradation of the stability with the size of the graph, we propose model (iii) of Prop.~\ref{prop:Delta}. In this model, where $\varepsilon$ measures the relative perturbation distance and $C$ the integral Lipschitz constant, the family of admissible perturbations has been restricted to those that satisfy the structural constraint \eqref{eqn:structuralConstraint}. Admissible perturbations are now those that are either dilations or contractions of the edge weights of $\bbS$. Dilations and contractions can be different for different nodes but cannot be a mix of dilation and contraction in different parts of the graph. We remark that if the structural constraint is satisfied, then the stability can be controlled by determining the integral Lipschitz constant of the filters, for any graph. However, for some specific families of graphs, where we have information on how the eigenvectors change with a given perturbation size, we can improve on the result by relaxing the structural constraint. This is the case of \cite{Mallat12-Scattering}, where extraneous geometric information (Euclidean space) is leveraged to quantify the impact of the perturbation (diffeomorphism) on the spectrum basis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{plots_stability/graph_dilation_unstable.tex}\medskip
    \input{plots_stability/graph_dilation_stable.tex}    
    \caption{Stability of graph filters. We observe that, for small values of $\lambda$, the difference between $\lambda_{i}$ (in blue) and $\hlam_{i}$ (in red) is small, whereas for large $\lambda$ this becomes much larger. (top) When using a Lipschitz filter [cf. \eqref{eqn:lipschitzFilters}], we observe that for low frequencies, the response of the filter is very similar when instantiated on either $\lambda_{i}$ or $\hlam_{i}$; however, for large frequencies, the difference becomes much larger, and thus a small change in the eigenvalues, leads to a big change of the filter response. (bottom) In the case of integral Lipschitz filters [cf. \eqref{eqn:integralLipschitzFilters}], the effect on high frequencies is mitigated, by forcing the filter to be nearly constant at these frequencies, so that, when evaluated at eigenvalues that are far away, the filter response is still almost the same, guaranteeing stability.}
    \label{fig_graph_dilation}
\end{figure}


%\begin{remark} \normalfont
%Theorem \ref{thm_filter_stability_structural_constraint} provides a bound that is independent of graph properties. An interesting consequence of this fact is that it makes it ready to take limits as we grow the number of nodes in the graph. There is, in fact, no limit to be taken as the bound holds for all graphs. Of particular importance is the limit of a line graph in which case we partially recover the seminal stability results for scattering transforms using regular convolutions in \cite{Mallat12-Scattering}. The difference between Theorem \ref{thm_filter_stability_structural_constraint} and the results in \cite{Mallat12-Scattering} is our restriction that the perturbation matrix be close to an identity. This means we can perturb the line graph by dilating all edges or by contracting all edges. Dilations and contractions can be different for different nodes but we cannot have a mix of dilation and contraction in different parts of the line. This is allowed in \cite{Mallat12-Scattering} where perturbations are arbitrary diffeomorphisms. The reason for the relative weakness of the result is that \cite{Mallat12-Scattering} leverages extrinsic geometric information that is not available in an analysis that applies to arbitrary graphs.
%\end{remark}
